Distributed Rumor Blocking with Multiple Positive Cascades

Misinformation and rumor can spread rapidly and widely through online social networks and therefore rumor controlling has become a critical issue. It is often assumed that there is a single authority whose goal is to minimize the spread of rumor by generating a positive cascade. In this paper, we study a more realistic scenario when there are multiple positive cascades generated by different agents. For the multiple-cascade diffusion, we propose the P2P independent cascade (PIC) model for private social communications. The main part of this paper is an analysis of the rumor blocking effect (i.e. the number of the users activated by rumor) when the agents non-cooperatively generate the positive cascades. We show that the rumor blocking effect provided by the Nash equilibrium will not be arbitrarily worse even if the positive cascades are generated non-cooperatively. In addition, we give a discussion on how the cascade priority and activation order affect the rumor blocking problem. We experimentally examine the Nash equilibrium of the proposed games by simulations done on real social network structures.

==> README <==

September 17, 2014


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8a has a number of significant changes over the v1.8 release.
For a full list of changes, please read the file changelog.txt. The most
notable changes include:


 1) Extensive rework of the compsoc mode to comply with the latest standards
    of the IEEE Computer Society.

 2) Fixed abstract, index terms and diamond line for compsoc technotes.

 3) New \IEEEraisesectionheading{} command to provide for the special
    raised first section heading of Computer Society journal papers.

 4) Internal code improvements for page setup and command argument
    processing.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> experiment_1.tex <==
\begin{table}[h]
\centering
{\begin{tabular}{ |p{0.8cm} | p{1.1cm}| p{1.1cm}| p{1.2cm} | p{1.2cm}| p{1.1cm} |}
\hline 
$B$& \small MBED & \small FBED& \small MLBED& \small OutDegree  \\ 
\hline
50	&   \textbf{46.32} &  47.54&   47.85	&  134.44\\
51	&   62.68 &  59.31&   \textbf{54.16}	&  134.53\\
52	&   \textbf{48.43} &  49.12&   89.96	&   64.78\\
53	&   77.54 &  70.85&   \textbf{59.88}	&    199.47\\
54	&   78.38 &  \textbf{64.05}&   69.36	&    126.47\\
55	&   68.24 &  \textbf{59.00}&   67.14	&    140.21\\
56	&   87.83 &  86.33&   \textbf{80.28}	&    168.81\\
57	&  	109.89 &  82.28&   \textbf{53.71}&    177.66\\
58	&   90.76 &  89.01&   \textbf{61.53}	&    152.14\\
59	&   92.15 &  \textbf{76.46}&   87.00	&    149.81\\
60	&   93.36 &  \textbf{82.84}&   88.07	&    157.98\\
61	&   60.62 &  60.18&   \textbf{59.55}	&    143.21\\
62	&   \textbf{56.79} &  59.34&   64.04	&    129.30\\
63	&  	230.67 & 226.27&  \textbf{181.02}&    131.62\\
64	&   67.46 &  70.41&   \textbf{61.29}	&    139.11\\
65	&  	102.13 &  90.29&   \textbf{72.90}&    199.98\\
66	&  	\textbf{131.22} & 149.62&  131.74&    162.81\\
67	&   88.95 &  89.35&   \textbf{77.79}	&    170.32\\
68	&   66.25 &  \textbf{64.72}&   65.89	&    143.20\\
69	&   77.82 &  \textbf{75.63}&  101.42	&    141.27\\
70	&   72.66 &  72.48&   \textbf{71.61}	&    130.33\\
71	&   70.88 &  73.65&   \textbf{69.56}	&    145.53\\
72	&   67.70&   \textbf{67.53}&   69.13&   234.21\\
73	&   \textbf{69.23}&  69.44 &  80.60 &   129.45\\
74	&   \textbf{68.43}&   69.88&   73.97&  158.98\\
75	&   \textbf{70.84}&	71.10&   72.26&    239.90\\
\hline
\end{tabular}}
\caption{\textbf{Table of Fig. \ref{fig:exp_1_uniform}} }
\label{table:experiment_1}
%\label{table:state1}
%\caption{States of edge $(v_{i,j},v_{0,i})$, for $i>0$.}
\end{table}






==> fig.tex <==









==> lambda.tex <==




\begin{table}[t]
\centering
{\begin{tabular}{ |p{0.6cm} | p{1.0cm}| p{1.0cm}| p{1.2cm} | p{1.4cm}| p{1.1cm} |}
\hline 
$\lambda$& \small MBED & \small FBED& \small MLBED& \small OutDegree &  \small Random \\  
\hline
0.05& \textbf{1.969} & 2.009 & 2.164  & 2.147& 2.287    \\

0.1& \textbf{2.767} & 3.062 &3.570 & 3.143 &  3.967   \\

0.15& 2.471 & 2.724 & 3.466 & \textbf{2.231} &  3.826 \\ 

0.2& 2.957 & 3.055  & 3.424  &\textbf{2.120}& 3.701  \\ 

0.25& \textbf{2.699} & 2.896 & 3.017 &2.721 & 3.264 \\ 

0.3& \textbf{3.377} & 3.447 & 3.744 & 3.761 & 5.102 \\

0.35& 1.657 & 1.767 & 1.882 & \textbf{1.321}& 2.894 \\

0.4& 2.598 & \textbf{2.478} & 3.063 & 2.673 & 3.347 \\

0.45& 2.077 & \textbf{2.008} & 2.016 & 2.103 & 2.332 \\

0.5& 3.592 & \textbf{3.467} & 4.541 & 4.230& 4.706 \\

0.55& 3.705 & 3.650 & \textbf{3.149} & 3.253 & 4.058 \\

0.6& 2.701 & 2.291 & 2.034 &\textbf{2.023} & 2.803 \\

0.65& 2.723 & 2.939 & 3.437 &\textbf{2.721}& 3.632 \\

0.70& 2.438 &\textbf{2.207} & 2.879  & 2.564 & 3.526 \\

0.75& \textbf{1.776} & 1.778 & 1.888 & 1.793 & 2.063 \\

0.80& 2.489 & \textbf{2.442} & 3.085 & 2.846 & 3.564 \\

0.85& 1.847 & \textbf{1.803} & 2.000 &1.963 & 2.241 \\

0.90& \textbf{1.911} & 2.103 & 1.924 &2.023 & 2.944 \\

0.95& 4.333 & \textbf{4.179} & 4.290 & 4.653 & 4.868 \\

%0.05& 1.9695 & 2.0093 & 2.4646  & 2.2872    \\

%0.1& 2.7677 & 3.0620 &3.5701 & 3.9672   \\

%0.15& 2.4719 & 2.7244 & 3.4669 & 3.8266 \\ 

%0.2& 2.9571 & 3.0554  &3.4242 & 3.7018  \\ 

%0.25& 2.6999 & 2.8967 & 3.6179 & 3.2640 \\ 

%0.3& 3.3778 & 3.4475 & 3.7445 & 5.1024 \\

%0.35& 1.6579 & 1.7674 & 1.8820 & 2.8946 \\

%0.4& 2.5989 & 2.4784 & 3.0635 & 3.3478 \\

%0.45& 2.0774 & 2.0080 & 2.5165 & 2.3325 \\

%0.5& 3.5927 & 3.4671 & 4.5415 & 4.7061 \\

%0.55& 3.7058 & 3.6504 & 4.1494 & 4.0586 \\

%0.6& 2.7011 & 2.2913 & 2.8341 & 2.8034 \\

%0.65& 2.7233 & 2.9391 & 3.4376 & 3.6327 \\

%0.70& 2.4384 & 2.2070 & 2.8796  & 3.5267 \\

%0.75& 1.7762 & 1.7788 & 2.2881 & 2.0638 \\

%0.80& 2.4896 & 2.4421 & 3.0854 & 3.5645 \\

%0.85& 1.8478 & 1.8034 & 2.3004 & 2.2413 \\

%0.90& 1.9112 & 2.1031 & 1.9240 & 2.9440 \\

%0.95& 4.3333 & 4.1791 & 4.2905 & 4.8680 \\
\hline
\end{tabular}}
\caption{\textbf{First experiment with $B=1$ under uniform setting.}  }
\label{table:B=1}
%\label{table:state1}
%\caption{States of edge $(v_{i,j},v_{0,i})$, for $i>0$.}
\end{table}

==> temp.tex <==
\begin{table}[t]
\centering
{\begin{tabular}{ |p{0.6cm} | p{1.0cm}| p{1.0cm}|p{1.1cm} | p{1.4cm}| p{1.2cm} |}
\hline 
$\lambda$& \small MBED & \small FBED& \small MLBED& \small OutDegree &  \small Random \\  
\hline
0.05& 33.311 & \textbf{23.513} & 35.062  & 32.004 & 104.142    \\

0.1& \textbf{23.513} & 24.903 &23.879 & 23.923 &  140.217  \\

0.15& \textbf{25.128} & 26.023 & 32.695 & 35.459 &  73.080 \\ 

0.2& 32.796 & 31.123  & 48.752  & \textbf{28.124} & 138.887 \\ 

0.25& \textbf{29.780} & 32.297 &32.155 & 34.678 & 95.753 \\ 

0.3& \textbf{26.742} & 35.655 & 29.161 &31.206 & 85.103 \\

0.35& 26.016 & \textbf{23.689} & 36.446 & 25.424 & 106.042 \\

0.4& 22.073 & 22.501 & \textbf{21.906} & 27.274 & 26.529\\

0.45& 25.814 & 22.833 & \textbf{22.096} & 28.853 & 24.225 \\

0.5& 29.431 & 28.444 & 34.897 & \textbf{25.055} & 85.988 \\

0.55& 47.988 & \textbf{47.416} & 58.054 & 50.102 & 145.812 \\

0.6& 31.002 & 30.991 & \textbf{28.703} & 53.519 & 83.826 \\

0.65& 37.392 & \textbf{36.734} & 45.628 & 38.692 & 120.187 \\

0.70& 49.401 & \textbf{46.954} & 47.607  & 62.775 & 64.513 \\

0.75& 28.583 & \textbf{27.240} & 35.064 & 33.419 & 113.668 \\

0.80& \textbf{30.373} & 31.695 & 30.660 & 54.396 & 54.380\\

0.85& 43.380 & 42.220 & \textbf{41.910} & 44.203 & 124.902 \\

0.90& 24.011 & \textbf{22.170} & 30.670 & 23.003 & 104.360 \\

0.95& 32.280 & \textbf{31.923} & 33.420 & 39.250 & 56.607 \\

%0.05& 1.9695 & 2.0093 & 2.4646  & 2.2872    \\

%0.1& 2.7677 & 3.0620 &3.5701 & 3.9672   \\

%0.15& 2.4719 & 2.7244 & 3.4669 & 3.8266 \\ 

%0.2& 2.9571 & 3.0554  &3.4242 & 3.7018  \\ 

%0.25& 2.6999 & 2.8967 & 3.6179 & 3.2640 \\ 

%0.3& 3.3778 & 3.4475 & 3.7445 & 5.1024 \\

%0.35& 1.6579 & 1.7674 & 1.8820 & 2.8946 \\

%0.4& 2.5989 & 2.4784 & 3.0635 & 3.3478 \\

%0.45& 2.0774 & 2.0080 & 2.5165 & 2.3325 \\

%0.5& 3.5927 & 3.4671 & 4.5415 & 4.7061 \\

%0.55& 3.7058 & 3.6504 & 4.1494 & 4.0586 \\

%0.6& 2.7011 & 2.2913 & 2.8341 & 2.8034 \\

%0.65& 2.7233 & 2.9391 & 3.4376 & 3.6327 \\

%0.70& 2.4384 & 2.2070 & 2.8796  & 3.5267 \\

%0.75& 1.7762 & 1.7788 & 2.2881 & 2.0638 \\

%0.80& 2.4896 & 2.4421 & 3.0854 & 3.5645 \\

%0.85& 1.8478 & 1.8034 & 2.3004 & 2.2413 \\

%0.90& 1.9112 & 2.1031 & 1.9240 & 2.9440 \\

%0.95& 4.3333 & 4.1791 & 4.2905 & 4.8680 \\
\hline
\end{tabular}}
\caption{ \textbf{Performance of the algorithms with $B=5$ under weighted cascade setting and $|X_1| \geq 20$.} }
\label{table:B=5}
\label{table:state1}
\end{table}



\begin{table}[h]
\centering
{\begin{tabular}{ |p{0.3cm} | p{1.1cm}| p{1.1cm}| p{1.2cm} | p{1.4cm}| p{1.1cm} |}
\hline 
$B$& \small MBED & \small FBED& \small MLBED& \small OutDegree & \small Random \\ 
\hline
%1 & \textbf{2.3340} & 3.0000 & 4.0930 & 2.2170 & 5.3090 \\

%2 & 5.063 & 4.459 & \textbf{4.286} & 5.486 & 10.248 \\

%3 & \textbf{8.121} & 8.310 & 9.343 & 9.997 & 10.844 \\ 

%4 & \textbf{22.773} & 24.389 & 23.910 & 23.120  & 30.598 \\ 

%5 & 24.553 & 23.810 & \textbf{23.231} & 26.563 & 35.868 \\

%6 & \textbf{37.235} & 37.365 & 35.303 & 38.864 & 38.561 \\

%7 & 30.182 & \textbf{28.682} & 31.793 & 32.627 & 35.209 \\

%8 & \textbf{9.425} & 17.007 & 17.807 &16.408 & 27.919 \\

%9 & 42.505 & 41.298 & \textbf{32.088} &40.418 & 48.421 \\

%10 & \textbf{29.261} & 30.392 & 31.882 & 30.079 & 32.815 \\

%11 & 23.448 & 22.291 & \textbf{19.914} & 24.498 & 25.493 \\

%12 & 15.601 & \textbf{14.883} & 22.332 & 14.543 & 30.001 \\

%13 & 29.609 & 29.333 & \textbf{25.253} & 28.627 & 32.522 \\

%14 & 28.442 & 28.550 & \textbf{27.917} & 30.771 & 35.144 \\

%15 & 5.367 & \textbf{4.912} & 6.194 &6.129 & 8.844 \\

%16 & 50.634 & 50.947 & \textbf{36.248} & 55.532 & 60.447 \\

%17 & \textbf{19.187} & 19.635 & 28.590 & 20.797 & 43.263 \\

%18 & 28.940 & 29.181 & \textbf{21.553} & 26.469 & 36.663 \\

%19 & 11.150 & 13.095 & 10.987 &\textbf{10.204} & 14.607 \\

20 & \textbf{20.48} & 21.62 & 20.67 & 23.44 & 24.54\\
21 &	38.36   &39.96   &23.30 &  87.80 & 120.96\\
22 &   18.08 &  18.25&  123.08  & 66.42 &  38.46\\
23	&  	61.19 &	56.22 &  33.93	&	92.48	&  	107.86\\
24	&	20.14 &	20.62 &  52.92	&	95.07 	& 	115.89\\
25	& 	45.97 &	48.94 &  30.33	& 	88.46 	& 	107.68 \\
26	& 	131.4 &	129.66&	153.96	&   43.34 &  	42.74\\
27	&	68.68 &	52.77 & 83.04  	& 126.99 & 128.75 \\
28	&  	171.78&	183.61&  129.68	&   76.09 &  45.05\\
29	&  	28.98 &	25.74 &  64.61	&   62.61 & 113.17 \\
30	&   75.18 & 74.06&   62.11	&  119.78&  148.05\\
31	&   27.23 & 27.53&   64.56	&   36.45&   48.81\\
32	&  	29.61 &	31.30 &  40.78 	& 101.71 & 108.52 \\
33	&  	125.19&	115.27&   41.52	&  105.77&  134.98\\
34	&  	59.09 & 65.71 &  50.48 	&  74.55 & 108.81\\
35	&   41.54 & 42.18&   40.29	&  104.46&  119.39\\
36	&   71.49 &  65.41&   71.14	&  128.36&  168.39\\
37	&   44.08 &  44.69&   39.41	&   82.81&  131.00\\
38	&   81.20 &  70.87&   79.66	&  107.88&  126.25\\
39	&   55.80 &  74.27&   46.33	&  131.02&  167.05\\
40	&  	121.96 & 132.09&   66.42	&   99.83&  106.22\\
41	&   37.29 &  38.45&   39.91	&   81.65&  140.22\\
42	&   42.05 &  41.87&   49.54	&  101.67&  132.49\\
43	&   40.10 &  40.73&   44.52	&   46.68&   57.54\\
44	&   76.73 &  52.23&   96.00	&  106.32&  126.44\\
45	&   71.41 &  65.40&   45.99	&  141.99&  148.14\\
46	&  	109.81 & 105.41&   59.21&  139.32&  162.11\\
47	&  	187.46 & 197.71&  196.77&  127.94&  125.94\\
48	&   52.65 &  49.73&   83.39	&   91.20&  128.45\\
49	&   49.54 &  46.95&   55.40	&   51.45&   54.79\\
50	&   46.32 &  47.54&   47.85	&   98.72&  134.44\\
%50	&   59.81 &  65.9900&   59.8100&  108.2640&  119.0700\\
51	&   62.68 &  59.31&   54.16	&  108.92&  134.53\\
52	&   48.43 &  48.12&   89.96	&   56.92&   64.78\\
53	&   77.54 &  70.85&   59.88	&  150.46&  199.47\\
54	&   78.38 &  64.05&   69.36	&  112.40&  126.47\\
55	&   68.24 &  59.00&   67.14	&  111.21&  140.21\\
56	&   87.83 &  86.33&   80.28	&  134.19&  168.81\\
57	&  	109.89 &  82.28&   53.71&  136.58&  177.66\\
58	&   90.76 &  89.01&   61.53	&  146.32&  152.14\\
59	&   92.15 &  76.46&   87.00	&  114.49&  149.81\\
60	&   93.36 &  82.84&   88.07	&  151.02&  157.98\\
61	&   60.62 &  60.18&   59.55	&  113.51&  143.21\\
62	&   60.79 &  59.34&   64.04	&  118.77&  129.30\\
63	&  	230.67 & 226.27&  181.02&  144.70&  131.62\\
64	&   67.46 &  70.41&   61.29	&  120.83&  139.11\\
65	&  	102.13 &  90.29&   72.90&  165.32&  199.98\\
66	&  	131.22 & 149.62&  131.74&  162.39&  162.81\\
67	&   88.95 &  89.35&   77.79	&  151.10&  170.32\\
68	&   66.25 &  64.72&   65.89	&  121.23&  143.20\\
69	&   77.82 &  75.63&  101.42	&  115.60&  141.27\\
70	&   72.66 &  72.48&   71.61	&  121.06&  130.33\\
71	&   70.88 &  73.65&   69.56	&  118.70&  145.53\\
72	&   67.70&   67.53&   69.13&  127.89 & 234.21\\
73	&   69.63&  69.44 &  80.60 &  91.44 & 129.45\\
74	&   70.43&   69.88&   73.97&  123.41& 158.98\\
75	&   70.84&	71.10&   72.26&  102.23&  239.90\\
\hline
\end{tabular}}
\caption{\textbf{Results of the first experiment under the uniform setting.} }
\label{table:experiment_1}
%\label{table:state1}
%\caption{States of edge $(v_{i,j},v_{0,i})$, for $i>0$.}
\end{table}





